Higher Order Estimating Equations for High-dimensional Models

We introduce a new method of estimation of parameters in semiparametric and nonparametric models. The method is based on estimating equations that are $U$-statistics in the observations. The $U$-statistics are based on higher order influence functions that extend ordinary linear influence functions of the parameter of interest, and represent higher derivatives of this parameter. For parameters for which the representation cannot be perfect the method leads to a bias-variance trade-off, and results in estimators that converge at a slower than $\sqrt n$-rate. In a number of examples the resulting rate can be shown to be optimal. We are particularly interested in estimating parameters in models with a nuisance parameter of high dimension or low regularity, where the parameter of interest cannot be estimated at $\sqrt n$-rate, but we also consider efficient $\sqrt n$-estimation using novel nonlinear estimators. The general approach is applied in detail to the example of estimating a mean response when the response is not always observed.

==> aad.tex <==
\catcode`\@=11 % allows @ to be used in control sequences in this format file

\newtheorem{assumption}{Assumption}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{example}{Example}[section]
\newcommand{\prf}{\begin{proof}{Proof}}
\newtheorem{remark}{Remark}[section]
%\renewcommand{\endproof}{\end{proof}}

\def\itemi{\item{(i)}}
\def\itemii{\item{(ii)}}
\def\itemiii{\item{(iii)}}
\def\itemiv{\item{(iv)}}
\def\itemv{\item{(v)}}
\def\itemvi{\item{(vi)}}


% Abbreviations
\def\A{{\cal A}} \def\a{{\alpha}}
\def\B{{\cal B}} \def\b{{\beta}}                        \def\BB{\mathbb{B}} \def\bB{{\bf B}}
\def\C{{\cal C}}                                        \def\CC{\mathbb{C}}
\def\D{{\cal D}} \def\d{{\delta}}     \def\gD{{\Delta}} \def\DD{\mathbb{D}}
                 \def\e{{\varepsilon}}                  \def\EE{\mathbb{E}} \def\bE{{\bf E}}
\def\F{{\cal F}} \def\f{{\phi}}                         \def\FF{\mathbb{F}}
\def\G{{\cal G}} \def\g{{\gamma}}                       \def\GG{\mathbb{G}}                           
\def\H{{\cal H}} \def\h{{\eta}}                         \def\HH{\mathbb{H}} \def\bH{{\bf H}}
\def\I{{\cal I}}                                        \def\II{\mathbb{I}} 
\def\J{{\cal J}}                                        \def\JJ{\mathbb{J}}              
\def\K{{\cal K}} \def\k{{\kappa}}                       \def\KK{\mathbb{K}}                              
\def\L{{\cal L}} \def\l{{\lambda}}    \def\gL{{\Lambda}}\def\LL{\mathbb{L}} \def\bL{{\bf L}}
\def\M{{\cal M}} \def\m{{\mu}}                          \def\MM{\mathbb{M}}
                 \def\n{{\nu}}                          \def\NN{\mathbb{N}}                              
\def\O{{\Omega}} \def\o{{\omega}}
\def\P{{\cal P}} \def\p{{\pi}}                          \def\PP{\mathbb{P}}
\def\Q{{\cal Q}} \def\q{{\theta}}                       \def\QQ{\mathbb{Q}}
\def\R{{\cal R}} \def\r{{\rho}}				\def\RR{\mathbb{R}}
                 \def\s{{\sigma}}     \def\S{{\Sigma}}  \def\SS{\mathbb{S}}
                 \def\t{{\tau}}       \def\T{{\Theta}}
\def\U{{\cal U}}					\def\UU{\mathbb{U}}
							\def\VV{\mathbb{V}}
\def\W{{\cal W}}                                        \def\WW{\mathbb{W}}
\def\X{{\cal X}} \def\x{{\xi}}				\def\XX{\mathbb{X}} \def\bX{{\bf X}}
\def\Y{{\cal Y}}					\def\YY{\mathbb{Y}} \def\bY{{\bf Y}}
\def\Z{{\cal Z}} \def\z{{\zeta}}                        \def\ZZ{\mathbb{Z}}


\def\sumin{{\sum_{i=1}^n}}
\def\sumjn{{\sum_{j=1}^n}}
\def\sumim{{\sum_{i=1}^m}}
\def\sumjm{{\sum_{j=1}^m}}
\def\sumik{{\sum_{i=1}^k}}
\def\sumjk{{\sum_{j=1}^k}}
\def\tsum{{\textstyle\sum\limits}}
\def\prodjn{{\prod_{j=1}^n}}
\def\prodin{{\prod_{i=1}^n}}
\def\prodim{{\prod_{i=1}^m}}
\def\prodjm{{\prod_{j=1}^m}}
\def\prodik{{\prod_{i=1}^k}}
\def\tprodik{\textstyle\prod_{i=1}^k\limits}
\def\tprod{{\textstyle\prod\limits}}
\def\prodm{\otimes} 
\def\prodmjn{{\bigotimes_{j=1}^n}}
\def\prodmin{{\bigotimes_{i=1}^n}}
\def\tprodmin{{\textstyle\bigotimes_{i=1}^n\limits}}
\def\tprodmjn{{\textstyle\bigotimes_{j=1}^n\limits}}
\def\tprodmim{{\textstyle\bigotimes_{i=1}^m\limits}}
\def\tprodmjm{{\textstyle\bigotimes_{j=1}^m\limits}}
\def\half{{\frac12}}
\def\thalf{{\textstyle\half}}
\def\tkwart{{\textstyle{\frac14}}}
\def\tint{{\textstyle\int\limits}}
\def\tbigcap{{\textstyle\bigcap\limits}}
\def\tbigcup{{\textstyle\bigcup\limits}}
\def\ra{\rightarrow}
\def\da{\downarrow}
\def\ua{\uparrow}
\def\dotfil{\leaders\hbox to 1em{\hss.\hss}\hfill}
\def\minqquad{\hskip-2em\relax}\def\minqqqquad{\hskip-4em\relax}
\def\qqqquad{\hskip4em\relax}\def\qqqqqquad{\hskip6em\relax}
\def\liminfsup{\mathop{\overline{\underline{\rm lim}}}}





% Mathematics
\def\hexnumber#1{\ifcase#1 0\or 1\or 2\or 3\or 4\or 5\or 6\or 7\or 8\or 9\or A\or B\or C\or D\or E\or F\fi}
%\mathchardef\boxminus="3\hexnumber\msafam0C
%\mathchardef\lesssim="3\hexnumber\msafam2E
%\mathchardef\gtrsim="3\hexnumber\msafam26
%\mathchardef\rightsquigarrow="3\hexnumber\msafam20
\def\mypartial#1{\mathchoice{\partial\over\partial#1}{\partial/\partial#1}{}{}}
\def\Re{\mathop{\rm Re}\nolimits}
\def\Im{\mathop{\rm Im}\nolimits}
\def\entier#1{\lfloor#1\rfloor}
\def\BL{{\rm B\kern -0.5pt L}}
\def\UC{{\rm U\kern-0.5pt C}}
\def\linfty{\ell^\infty}
\def\simplex{{\rm S}}
\def\id{id}
\def\argmax{\mathop{\rm argmax}}
\def\argmin{\mathop{\rm argmin}}
\def\trace{{\rm trace }}
\def\diag{\mathop{\rm diag\,}\nolimits}
\def\lin{\mathop{\rm lin\,}\nolimits}
\def\closedlin{\overline{\lin}}
\def\tanh{\mathop{\rm tanh}\nolimits}
\def\arctanh{\mathop{\rm arctanh}\nolimits}
\def\arctg{\mathop{\rm arctg}\nolimits}
\def\loglog{\mathop{\rm loglog}\nolimits}
\def\sign{\mathop{\rm sign}\nolimits}
%\def\interior{{\rm int}}
\def\interior{\mathaccent 23}
\def\closure#1{\overline{#1}}
\def\boundary{\mathop{\delta}\nolimits}
\def\closedhull{{\overline{\hull}}}
\def\closedconv{\closedhull}
\def\essinf{\mathop{\rm essinf}\limits}
\def\conv{\hull}
\def\hull{\mathop{\rm conv\ }\nolimits}
\def\diam{\mathop{\rm diam}\nolimits}
\def\ball{\mathop{\rm ball}\nolimits}
\def\closedball{\overline{\ball}}
\def\every{\hbox{ every }}
\def\forevery{\hbox{ for every }}
\def\OR{\hbox{ or }}
\def\implies{\hbox{ $\Rightarrow$ }}
\def\seilpmi{\hbox{ $\Leftarrow$ }}
\def\bydef{\buildrel {\rm def}\over =}
\def\qed{\ \vrule height4pt width4pt depth0pt}
\def\halmos{\ \vbox{\hrule\hbox{\vrule\vbox{\phantom{\vrule height4pt width4pt depth0pt}}\vrule}\hrule}}

% Statistics
\def\Prodint{\mathop{\mathchoice{\vcenter{\epsfysize=1.5em\epsfbox{%
  prodint.eps}}}{\vcenter{\epsfysize=1em\epsfbox{prodint.eps}}}{}{}}}
\def\prodint{\Prodint}
\def\tdot#1{\kern1.2pt\dot{\vphantom{#1}}\kern-1.2pt
        \dot#1\kern0.8pt\dot{\vphantom{#1}}\kern-0.8pt}
\def\contiguous{\triangleleft}
\def\doublecontiguous{\mathrel{\triangleleft\,\joinrel\triangleright}}
\def\E{\mathord{\rm E}}
\def\Pr{\mathord{\rm P}}
\def\var{\mathop{\rm var}\nolimits}
\def\sdev{\mathop{\rm sd}\nolimits}
\def\cov{\mathop{\rm cov}\nolimits}
\def\Cov{\mathop{\rm Cov}\nolimits}
\def\cor{\mathop{\rm cor}\nolimits}
\def\Cor{\mathop{\rm Cor}\nolimits}
\let\covar\cov
\let\Covar\Cov
\let\Var=\var
\def\med{\mathop{\rm med}\nolimits}
\def\medlimits{\mathop{\rm med}\limits}
\def\almostsurely{{\rm a.s.}}
\def\almosteverywhere{{\rm a.e.}}
\def\infinitelyoften{{\rm i.o.}}
\def\ae{\almosteverywhere}
\def\ldot{\hbox {$\dot \ell$}}
\def\ltil{\hbox{$\tilde \ell$}}
\def\dirac{\delta}
\def\haslaw{\sim}
\def\haslawunder#1{\mathchoice{\buildrel #1\over \sim}{\ \mathrel{^{#1}}\joinrel\sim}{}{}}
\def\generatedby{\s}
\mathchardef\given="626A
\mathcode`:="603A
%\mathchardef\setminus="2200


% Convergence symbols
\def\generalweak#1{\ {\mathchoice{\buildrel #1\over \rightsquigarrow}%
{\raise-2pt\hbox{$\buildrel #1\over \rightsquigarrow$}}{}{}}\ }
\let\weak\rightsquigarrow
\def\generalprob#1{\ {\mathchoice{\raise-1.5pt\hbox{$\buildrel#1\over\ra$}}
{\raise-2pt\hbox{$\buildrel#1\over\ra$}}{}{}}\ }
\def\outerp{\generalprob {\small P*}}
\def\prob{\generalprob{\small P}}
\def\outeras{\generalprob{\small as*}}
\def\as{\generalprob{\small as}}
\def\vague{\generalprob{\small v}}
\def\au{\generalprob{\small au}}
\def\Pgg{\ {\mathchoice{\raise-1.5pt\hbox{$\buildrel {\small P}\over\gg$}}
{\raise-2pt\hbox{$\buildrel {\small P}\over\gg$}}{}{}}\ }

% Miscellaneous
\def\beginskip{\begingroup\long\def\eet##1\endskip{\endgroup}\eet}
\def\endskip{}
\def\boxit#1{\vbox{\hrule\hbox{\vrule\kern1pt\vbox{\kern1pt #1\kern1pt}\kern1pt\vrule}\hrule}}
\def\eet#1{}
\def\makenumbersactive{\catcode`\0=11\catcode`\1=11\catcode`\2=11%
        \catcode`\3=11\catcode`\4=11\catcode`\5=11%
        \catcode`\6=11\catcode`\7=11\catcode`\8=11\catcode`\9=11 }



\catcode`\@=12







